Quantum Optimization Methods for the Generalized Traveling Salesman Problem

This paper studies quantum optimization baselines for the Generalized Traveling Salesman Problem (GTSP), a clustered routing problem that naturally models variant selection and sequencing problems under discrete alternatives. We propose a novel GTSP QUBO formulation focused on maintaining feasible solutions for quantum annealing, as well as a hardware-executable gate-based pipeline utilizing the Quantum Approximate Optimization Algorithm (QAOA). We implement a constrained QAOA variant using an XY-mixer, which preserves the stepwise Hamming weight in the ideal circuit model, while feasibility with respect to the full GTSP constraints is tracked explicitly during post-processing. We compare the two quantum optimization paradigms on problem instances from GTSPLIB, an established benchmark dataset, and validate against classical state-of-the-art solvers. To mitigate current quantum hardware size limitations, we further extend a preprocessing method to reduce the node count in instance clusters, constructing new NISQ-friendly instances from reduced subsets. Across all tested instances, quantum solvers often produce competitive solution quality when tested on smaller graphs, but exhibit higher runtimes and a sharp degradation in feasibility and scalability as instance size grows. Our evaluation highlights where quantum optimizers can already succeed and which algorithmic bottlenecks, like sampling rates, runtime issues, and other practical failure modes, remain as open problems.

==> tikz/circuit.tex <==
\iffalse
\begin{quantikz} % For a tutorial on quantikz, see http://mirrors.ibiblio.org/CTAN/graphics/pgf/contrib/quantikz/quantikz.pdf
 \lstick{$\ket{0}$} \qw & \gate{H} & \ctrl{4}  & \qw  & \qw & \qw & \gate[wires=4]{QFT^\dagger}  &    \rstick{$\ket{\phi_1}$} \qw \\
 \lstick{$\ket{0}$} \qw &  \gate{H} & \qw & \ctrl{3}  & \qw  & \qw  & \qw &  \rstick{$\ket{\phi_2}$}\qw \\
  \lstick{$\vdots$} & &  &  &  \ \ldots\  & &  & \rstick{$\vdots$}\qw \\
 \lstick{$\ket{0}$} \qw  & \gate{H} & \qw & \qw  & \qw & \ctrl{1}   & \qw &  \rstick{$\ket{\phi_m}$}\qw \\
 \lstick{$\ket{\varphi_i}$} \qw & \qw & \gate{U}  & \gate{U^2}   & \ \ldots\ \qw &  \gate{U^{2^{m-1}}}  & \qw  & \rstick{$\ket{\varphi_i}$}\qw 
\end{quantikz}
\fi


\begin{quantikz}[row sep=0.6cm, column sep=0.5cm]
\lstick{$q_0$} & \gate{H} & \ctrl{1} & \qw & \ctrl{2} & \qw & \gate{R_Z(\gamma \lambda)} & \gate{R_X(2\beta)} & \meter{} \\
\lstick{$q_1$} & \gate{H} & \ctrl{-1} & \ctrl{1} & \qw & \qw & \gate{R_Z(\gamma \lambda)} & \gate{R_X(2\beta)} & \meter{} \\
\lstick{$q_2$} & \gate{H} & \qw & \ctrl{-1} & \ctrl{1} & \qw & \gate{R_Z(\gamma \lambda)} & \gate{R_X(2\beta)} & \meter{} \\
\lstick{$q_3$} & \gate{H} & \qw & \qw & \ctrl{-1} & \qw & \gate{R_Z(\gamma \lambda)} & \gate{R_X(2\beta)} & \meter{}
\end{quantikz}



==> txt/8_Future-Work.tex <==
\iffalse
\textcolor{red}{TODO: Significantly shorten this section and add as a part of the conclusion}
In our experiments, we were able to achieve solution qualities comparable to classical solvers, but only for smaller problem instances. However, it became clear that for larger instances our approaches, together with the limitations of current quantum hardware, were usually not able to find feasible solutions anymore. In addition, the required quantum computation time increased significantly with growing problem size. These observations indicate that scalability remains a major challenge for quantum approaches to the GTSP.
Based on the insights gained during this work, we developed the idea of a hybrid, edge-based encoding approach combined with a problem-specific embedding, a concept, which opens several promising directions for future research. In particular, we identified three approaches that could contribute to improving performance in future work.
\subsection{LP-Reduced-Cost Elimination}
First, LP-reduced-cost elimination could be used as a classical preprocessing step to reduce the problem size while still preserving the optimal tour. This technique has already shown strong results for the TSP~\cite{cook2024local}, where it can reduce dense graphs with $O(n^2)$ edges to sparse graphs with only around $5n$ to $11n$ edges, without removing any optimal solutions. Transferring this idea to the GTSP by using a cluster-aware LP relaxation could significantly shrink the search space, especially for larger instances. Such a reduction would also make subsequent quantum encoding and embedding steps considerably easier.
\subsection{Edge-Based Encoding}
Second, an edge-based encoding could be applied to further reduce the number of required qubits. Madhu et al.~\cite{madhu2025edge} showed that compared to node-based encodings, edge-based approaches reduce the qubit complexity from $O(n^2)$ to $O(n \log n)$. For the GTSP, this encoding is particularly suitable, since exactly one node per cluster has to be selected. By focusing on inter-cluster edges and enforcing cluster constraints via penalties, the solution space can be reduced from (n!) city permutations to only $m!$ cluster permutations, where $m \ll n$. This could allow significantly larger GTSP instances to be tackled on near-term quantum hardware.
\subsection{Problem-Specific Embedding}
Third, we propose the development of a problem-specific embedding that explicitly exploits the cluster structure of the GTSP. Previous work~\cite{gomez2025addressing}  has shown that embedding quality has a strong influence on the success of quantum annealing, with long qubit chains leading to substantially worse results. Generic embedding tools such as Minorminer often struggle with the dense graph structures arising from TSP and GTSP formulations. A GTSP-specific embedding strategy could, for example, pre-place clusters using force-directed layouts, prioritize high-weight inter-cluster edges, and use clique-based embeddings for cluster connections. 

Overall, these three ideas naturally complement each other. LP-reduced-cost elimination simplifies the problem graph, edge-based encoding minimizes qubit requirements, and problem-specific embeddings improve the hardware mapping. Combined into an integrated pipeline, this approach could make it possible to solve larger GTSP instances on today’s quantum processors, where individual methods alone are not sufficient.
It should be emphasized that the integrated approach described above was not intended to be implemented within this work from the beginning. The idea for such a hybrid framework emerged gradually during the course of the research, based on the insights gained while developing and evaluating the presented methods. As a result, it remained a conceptual contribution rather than an implementation goal of this thesis.
Nevertheless, we believe that each of the proposed ideas has clear potential, and that bringing these ideas together could open new directions for solving the GTSP using quantum hardware. We hope that the insights gained in this work, as well as the outlined concepts, can serve as inspiration for future research and encourage others to further explore and possibly implement parts of these ideas.
\fi


